Using Gradient to Boost the Generalization Performance of Deep Learning Models for Fluid Dynamics

Nowadays, Computational Fluid Dynamics (CFD) is a fundamental tool for industrial design. However, the computational cost of doing such simulations is expensive and can be detrimental for real-world use cases where many simulations are necessary, such as the task of shape optimization. Recently, Deep Learning (DL) has achieved a significant leap in a wide spectrum of applications and became a good candidate for physical systems, opening perspectives to CFD. To circumvent the computational bottleneck of CFD, DL models have been used to learn on Euclidean data, and more recently, on non-Euclidean data such as unstuctured grids and manifolds, allowing much faster and more efficient (memory, hardware) surrogate models. Nevertheless, DL presents the intrinsic limitation of extrapolating (generalizing) out of training data distribution (design space). In this study, we present a novel work to increase the generalization capabilities of Deep Learning. To do so, we incorporate the physical gradients (derivatives of the outputs w.r.t. the inputs) to the DL models. Our strategy has shown good results towards a better generalization of DL networks and our methodological/ theoretical study is corroborated with empirical validation, including an ablation study.

==> Configs/FirstPage.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%           First Page  		         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\def\@engschool{engschool}
\newcommand{\engschool}[1]{
  \def\@engschool{#1}
}

\def\@specialty{specialty}
\newcommand{\specialty}[1]{
  \def\@specialty{#1}
}

\def\@director{director}
\newcommand{\director}[1]{
  \def\@director{#1}
}

\def\@advisor{advisor}
\newcommand{\advisor}[1]{
  \def\@advisor{#1}
}
\def\@jurya{}{}{}
\newcommand{\jurya}[3]{
  \def\@jurya{#1,	& #2	& #3\\}
}
\def\@juryb{}{}{}
\newcommand{\juryb}[3]{
  \def\@juryb{#1,	& #2	& #3\\}
}
\def\@juryc{}{}{}
\newcommand{\juryc}[3]{
  \def\@juryc{#1,	& #2	& #3\\}
}

\makeatother

\newcommand\BackgroundPic{%
	\put(0,0){%
		\parbox[b][\paperheight]{\paperwidth}{%
			\includegraphics[height=0.45\paperheight,width=0.1\textwidth]{Configs/AI.png}%
			\vfill
		}
	}
}
\newcommand\EtiquetteThese{%
	\put(0,0){%
		\parbox[t][\paperheight]{\paperwidth}{%
			\hfill
			\colorbox{blue}{		
				\begin{minipage}[b]{3em}
					\centering\Huge\textcolor{white}{MS\\H\\P\\C\\AI\\}
					\vspace{0.2cm}
				\end{minipage}
			}
		}
	}
}

\makeatletter
\newcommand{\firstpage}{
\newgeometry{top=1cm, bottom=2cm, left=2cm, right=1cm}
\AddToShipoutPicture*{\BackgroundPic}
\AddToShipoutPicture*{\EtiquetteThese}
  \begin{titlepage}
  \centering
      \includegraphics[width=0.15\textwidth]{Configs/Mines.pdf}
      \hfill
      \includegraphics[width=0.2\textwidth]{Configs/logo-psl.jpg}\\
    \vspace{1cm}
      {\Large Mastère Spécialisé: HPC and Artificial Intelligence for Industry}\\
    \vspace{1cm}
      {\Large 
      	%{\bfseries Mines ParisTech}\\
    \vspace{0.5cm}
      	ADVANCED MASTER'S THESIS }\\
    %\vfill
     %  {\LARGE \color[rgb]{0,0,1} \bfseries{\@title}} \\
    %\vfill
     \vspace{1cm}
   		\textit{prepared at}\\
    \vspace{1cm}
    	{\Large\bfseries \@engschool \, \&\, Extrality}\\
    \vspace{1cm}
    	\textit{presented and defended by}\\
    \vspace{0.5cm}
    	{\Large {\bfseries {\@authname} {\@authsurn}}} \\
    \vspace{0.5cm}
    	 \@date \\
    \vfill
       {\LARGE \color[rgb]{0,0,1} \bfseries{\local@title}} \\
    \vfill
    \begin{tabular}{llr}
		  \large {\it Supervisors} &\\
          \textbf{\@director{}} & Mines ParisTech\\
         \small \textit{ Professor/Director Post Master HPC-AI} &\\
         \textbf{\@advisor{}} & Extrality\\
         \small \textit{Machine Learning team lead} &\\
    \end{tabular}
    \vfill
	\begin{tabular}{>{\bfseries}llr}
		%\large {\it Graduation commitee}\\
		\@jurya{}
		\@juryb{}
		\@juryc{}
	\end{tabular}
	\vfill
	
	\textbf{MINES ParisTech | PSL University\\
	F-06904 Sophia Antipolis, France}
  \end{titlepage}


\restoregeometry  
  
  
}
\makeatother
